ReDel: A Toolkit for LLM-Powered Recursive Multi-Agent Systems

Recently, there has been increasing interest in using Large Language Models (LLMs) to construct complex multi-agent systems to perform tasks such as compiling literature reviews, drafting consumer reports, and planning vacations. Many tools and libraries exist for helping create such systems, however none support recursive multi-agent systems -- where the models themselves flexibly decide when to delegate tasks and how to organize their delegation structure. In this work, we introduce ReDel: a toolkit for recursive multi-agent systems that supports custom tool-use, delegation schemes, event-based logging, and interactive replay in an easy-to-use web interface. We show that, using ReDel, we are able to easily identify potential areas of improvements through the visualization and debugging tools. Our code, documentation, and PyPI package are open-source and free to use under the MIT license at https://github.com/zhudotexe/redel.

==> drafts/old_experiments.tex <==
\section{Experimental Setup}
\label{sec:experiments}
To validate the ReDel system and demonstrate how it can be used to run different systems, we test 8 system configurations on 3 benchmarks. We include the logs of each run in our attached code release and release our source code\footnote{\url{https://github.com/zhudotexe/redel/tree/demo/emnlp}} to enable reproduction and to load each experiment in the ReDel web interface. 

\paragraph{System Configuration.}
We test three main variables in how we configure systems to compare multi-agent recursive delegation systems with single-agent baseline systems, show how smaller models can be used in conjunction with larger models, and show how recursive delegation can enable shorter-context models to complete long-horizon tasks. For each system, we use GPT-4o (\texttt{gpt-4o-2024-05-13}; \citet{gpt-4o}) and/or GPT-3.5-turbo (\texttt{gpt-3.5-turbo-0125}\footnote{\url{https://platform.openai.com/docs/models/gpt-3-5-turbo}}) with 0 temperature for decoding.


% trim this for findings paper if need room?
\begin{enumerate}
    \item \textbf{Impact of delegation.} We compare two recursive delegation systems, \textit{RD-Full} and \textit{RD-Root-Tools}, against a single-agent baseline, \textit{SA-Base}. All root and delegate models use GPT-4o with 128k context length. \textit{RD-Full}'s root node does not have the ability to call tools other than the provided delegation scheme; \textit{RD-Root-Tools} was provided both delegation tools and each benchmark's tools and was responsible for choosing which tool to use.
    \item \textbf{Delegate model size.} We compare a system where a stronger model, GPT-4o, is responsible for delegating tasks to smaller models (i.e., GPT-3.5-turbo; \textit{RD-Small-Del}) to a system where every node is powered by the small model (\textit{RD-Small-All}). We also test a single-agent system as a baseline using the smaller model (\textit{SA-Small}).
    \item \textbf{Model context length.} Finally, we artificially limit GPT-4o's context length to 8192 tokens, and compare a recursive delegation system (\textit{RD-Short}) to a single-agent baseline system (\textit{SA-Short}).
\end{enumerate}

\paragraph{Benchmarks.}
We test these systems on three benchmarks:

\begin{enumerate}
    \item \textbf{FanOutQA} \cite{zhu2024fanoutqamultihopmultidocumentquestion}. FanOutQA is an information-seeking benchmark involving questions that require agents to collate information from multiple Wikipedia articles to answer a top-level question. The Open Book setting provides models with tools to search Wikipedia and models must perform long-horizon multi-hop reasoning to find the final answer across multiple articles.
    \item \textbf{TravelPlanner} \cite{xie2024travelplanner}. TravelPlanner tests agents' planning capabilities with natural language queries of varying difficulties requesting constrained travel plans. Agents must use provided tools to search flight, restaurant, and attraction databases to return a plan that meets both the explicitly defined constraints and commonsense constraints.
    \item \textbf{WebArena} \cite{zhou2024webarena}. WebArena presents agents with a realistic web environment, in which they must perform a diverse set of web tasks using tools to interact with a browser. These tasks take many rounds of interaction and range from adding products to a shopping cart to commenting on a GitLab issue and beyond.
\end{enumerate}

We tabulate these system configurations and compare the benchmarks used in Appendix \ref{sec:experiment_configs}.


\begin{table}
\centering
\small
\begin{tabular}{l|ccc}
\toprule
\textbf{System} & \textbf{FOQA} & \textbf{TP} & \textbf{WA} \\
\midrule
RD-Full         & \textbf{0.494} & \textbf{2.778} & \textbf{0.203} \\
RD-Root-Tools   & 0.429          & 0              & 0.188 \\
SA-Base         & 0.394          & 0              & 0.162 \\
\midrule
RD-Small-Del    & 0.255          & 0.556          & 0.122 \\
RD-Small-All    & 0.087          & 0              & 0.092 \\
SA-Small        & 0.077          & 0              & 0.085 \\
\midrule
RD-Short        & 0.426          & ---            & 0.129 \\
SA-Short        & 0.361          & ---            & 0.122 \\
\bottomrule
\end{tabular}
\caption{Systems' performance on FanOutQA (FOQA; Model Judge reported), TravelPlanner (TP; Final score reported), and WebArena (WA; Success Rate reported).}
\label{tab:results}
\end{table}

\section{Results \& Discussion}
In every benchmark, recursive delegation systems significantly outperform single-agent systems in almost all metrics.
Table \ref{tab:results} lists the primary metrics of each benchmark; we break down the systems' performance per-benchmark in Appendix \ref{sec:detailed_results}. We find two main failure cases in recursive systems, which we call \textbf{overcommitment} and \textbf{undercommitment}.

Overcommitment is most prevalent in systems where the root node has access to tools; it refers to the case where instead of decomposing and delegating tasks, the root node attempts to complete the top-level task itself. This is most visible in the FanOutQA and TravelPlanner benchmarks. In these benchmarks, the model performs multiple tool call rounds, filling its context window with retrieved information, leading to failures to complete the original task due to the retrieved information truncating the original task from its context. Comparing the \textit{SA-Base} and \textit{RD-Root-Tools} systems in these benchmarks, we see that simply providing the root model with delegation tools only results in a small or no improvement in end-to-end performance (0-10\%). In the ReDel web interface, this manifests as an abnormally small computation graph, often consisting of only a single node.

In contrast, undercommitment refers to a model performing no work and only re-delegating the task it was given. In all three benchmarks, this led to failure as models entered an infinite loop of delegation until it reached a query timeout. In the ReDel web interface, this manifests as a line of nodes in the computation graph (Figure \ref{fig:undercommitment}).

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\columnwidth]{img/undercommitment.pdf}
    \caption{Recursive systems exhibiting undercommitment produce long chains of agents (blue boxes), as seen in the ReDel computation graph.}
    \label{fig:undercommitment}
\end{figure}

We also find that recursive delegation can be used to improve systems of small models by using a single larger model as a task dispatcher. Comparing the \textit{RD-Small-Del} system to \textit{RD-Small-All} and \textit{SA-Small}, we find that although a recursive system comprised entirely of small models outperforms a single small-model agent, using a larger model as the root node produces a far greater performance gain. Though the \textit{RD-Small-Del} system still underperforms compared to the large-model \textit{SA-Base}, it is useful for optimizing for cost, as less tokens are sent to the larger (and more expensive) model. Using ReDel to count tokens from the event files of these systems (as demonstrated in Figure \ref{fig:event_usage}), we find that the \textit{SA-Base} system on average costs 178\% more than the \textit{RD-Small-Del} system, while only performing 33-54\% better.

Finally, we see that recursive delegation improves models with shorter contexts' performance on long-context tasks.

As this paper is focused on the ReDel system demonstration rather than models' performance, we plan to investigate these findings further in a future follow-up work.


\section{Detailed Results}
\label{sec:detailed_results}

This is a mess. Sorry.

\begin{table}[h]
\tiny
\centering
\begin{tabular}{l|ccccccc||l|ccc}
\toprule
& \multicolumn{7}{c||}{\textbf{FanOutQA}} & & \multicolumn{3}{c}{\textbf{WebArena}} \\
\textbf{System Key} & \textbf{Loose} & \textbf{Strict} & \textbf{ROUGE-1} & \textbf{ROUGE-2} & \textbf{ROUGE-L} & \textbf{BLEURT} & \textbf{Model Judge} & \textbf{System Key} & \textbf{SR} & \textbf{SR (AC)} & \textbf{SR (UA)} \\
\midrule
full         & \textbf{0.687} & \textbf{0.229}  & \textbf{0.321} & \textbf{0.175} & \textbf{0.289} & \textbf{0.511}  & \textbf{0.494} & full         & \textbf{0.203} & \textbf{0.179} & 0.643 \\
root-fc   & 0.658          & 0.190           & 0.302          & 0.158          & 0.272          & 0.508           & 0.429          & root-fc   & 0.188 & 0.171 & 0.500 \\
baseline         & 0.650          & 0.174           & 0.278          & 0.144          & 0.249          & 0.508           & 0.394          & baseline         & 0.162 & 0.128 & \textbf{0.786} \\
\midrule  
small-leaf    & 0.551          & 0.129           & 0.247          & 0.127          & 0.219          & 0.487           & 0.255          & small-leaf    & 0.122 & 0.109 & 0.357 \\
small-all    & 0.300          & 0.039           & 0.134          & 0.061          & 0.118          & 0.427           & 0.087          & small-all    & 0.092 & 0.066 & 0.571 \\
small-baseline        & 0.275          & 0.035           & 0.128          & 0.053          & 0.111          & 0.454           & 0.077          & small-baseline        & 0.085 & 0.058 & 0.571 \\
\midrule  
short-context        & 0.654          & 0.190           & 0.306          & 0.161          & 0.272          & 0.501           & 0.426          & short-context        & 0.129 & 0.105 & 0.571 \\
short-baseline        & 0.613          & 0.161           & 0.224          & 0.108          & 0.198          & 0.503           & 0.361          & short-baseline        & 0.122 & 0.093 & 0.643 \\
\bottomrule
\end{tabular}

\begin{tabular}{l|cccccc}
& \multicolumn{6}{c}{\textbf{TravelPlanner}} \\
\textbf{System Key} & \textbf{Delivery Rate} & \textbf{CS Micro} & \textbf{CS Macro} & \textbf{Hard Micro} & \textbf{Hard Macro} & \textbf{Final} \\
\midrule  
full         & 97.778 & \textbf{67.847} & \textbf{3.889} & 9.524  & 7.778\tablefootnote{Recursive systems tend to make more commonsense inputs for meals (e.g. ``on the flight'' or ``packed lunch'') -- this causes the evaluation script to give a score of 0 on the Hard Constraint metrics.}  & \textbf{2.778} \\
root-fc   & 71.667 & 46.944 & 0.000 & 15.714 & 11.111 & 0.000 \\
baseline         & 77.778 & 50.833 & 0.556 & \textbf{18.810} & \textbf{11.667} & 0.000 \\
\midrule  
small-leaf    & 97.222 & 65.903 & 0.556 & 2.143  & 1.111  & 0.556 \\
small-all    & \textbf{98.889} & 54.583 & 0.000 & 0.000  & 0.000  & 0.000 \\
small-baseline        & 88.889 & 48.750 & 0.000 & 0.238  & 0.000  & 0.000 \\
\bottomrule
\end{tabular}

\caption{Breakdown of results for each of the 3 tested benchmarks, divided by benchmark.}
\label{tab:detailed_results}
\end{table}
